Adversarial Risk and Robustness: General Definitions and Implications for the Uniform Distribution

We study adversarial perturbations when the instances are uniformly distributed over $\{0,1\}^n$. We study both "inherent" bounds that apply to any problem and any classifier for such a problem as well as bounds that apply to specific problems and specific hypothesis classes. As the current literature contains multiple definitions of adversarial risk and robustness, we start by giving a taxonomy for these definitions based on their goals, we identify one of them as the one guaranteeing misclassification by pushing the instances to the error region. We then study some classic algorithms for learning monotone conjunctions and compare their adversarial risk and robustness under different definitions by attacking the hypotheses using instances drawn from the uniform distribution. We observe that sometimes these definitions lead to significantly different bounds. Thus, this study advocates for the use of the error-region definition, even though other definitions, in other contexts, may coincide with the error-region definition. Using the error-region definition of adversarial perturbations, we then study inherent bounds on risk and robustness of any classifier for any classification problem whose instances are uniformly distributed over $\{0,1\}^n$. Using the isoperimetric inequality for the Boolean hypercube, we show that for initial error $0.01$, there always exists an adversarial perturbation that changes $O(\sqrt{n})$ bits of the instances to increase the risk to $0.5$, making classifier's decisions meaningless. Furthermore, by also using the central limit theorem we show that when $n\to \infty$, at most $c \cdot \sqrt{n}$ bits of perturbations, for a universal constant $c< 1.17$, suffice for increasing the risk to $0.5$, and the same $c \cdot \sqrt{n} $ bits of perturbations on average suffice to increase the risk to $1$, hence bounding the robustness by $c \cdot \sqrt{n}$.

==> AttacksGeneric.tex <==
\subsection{Generic  Bounds on Adversarial Risk and Robustness}
In this section we show how to use known results from the context of cryptographic attacks on coin tossing protocols \cite{lichtenstein1989some} and other primitives \cite{mahloujifar2017blockwise,mahloujifar2017learning} to obtain generic attacks on the robustness and risk under the uniform distribution, or more generally product distributions. We start by defining the metric under which these attacks are obtained; namely the Hamming distance.

\begin{definition}
For any product set  $\cZ=\cZ_1\times \dots \times \cZ_n$ the  Hamming distance $\BHD: \cZ\times\cZ \to \N$ is defined as
$\BHD(z,z') = \left|\{i\in [n] \colon z_i \neq z'_i\}\right|$  where  $z=(z_1,\dots,z_n), z'=(z'_1,\dots,z'_n), z_i,z_i' \in \cZ_n$.
\end{definition}

The following result of \cite{lichtenstein1989some} gives an upper bound on the number of corruptions needed for flipping the output of any coin tossing protocol.

\begin{theorem}\cite{lichtenstein1989some} \label{thm:linial}
For any function $f\colon\{0,1\}^n \to \{0,1\}$, if $\mu = \Ex_{x \gets U_n}[f(x)]$, then
     $\expectedsub{x\in\{0,1\}^n}{\min \set {r \colon \exists x' \in \HD_r(x), f(x')=1}}$ is $ O(\sqrt{- n \log \mu})$
     where $\HD$ is the binary Hamming distance. 
\end{theorem} 

The following corollary directly follows  from the definition of error-region adversarial risk, 
given in Definition \ref{def:ER}, and Theorem \ref{thm:linial} above.
\begin{corollary} \label{cor:robustness}
Suppose $\problem=(\X,\Y,\D,\C,\hypoC,\loss)$ is a classification problem with corresponding Boolean $\loss$ function. For  and any $h \in \H, c\in \C $, we have
\begin{displaymath}
\rho\eDR_{\HD,1}(h,U_n,c) \leq O\left(\sqrt{-n\cdot \log(\Risk(h,U_n,c))}\right)\,.
\end{displaymath}
\end{corollary}

Corollary \ref{cor:robustness} shows that for any constant $\mu = \log(\Risk(h,U_n,c)$ for a problem of dimension $n$ and \emph{uniform} input distribution,  the adversarial disagreement region risk  is always \emph{sublinear} over the dimension. The down side of this attack is that it is purely information theoretic, as it cannot be implemented in polynomial time; namely, it only shows the \emph{existence} of a close $x'$ that is misclassified. 

We now describe another set of tools from \cite{mahloujifar2017blockwise,mahloujifar2017learning} that can be used to increase the adversarial \emph{risk} under the more general setting where the input distribution is a \emph{product} distribution (perhaps over larger alphabets). The crucial property of these attacks is that, they could be implemented in polynomial time, given access to certain information about $h,c$. 

\begin{definition} [Tampering algorithm]
For any product set $\cZ= \cZ_1\times \dots \times \cZ_n$ we call an algorithm $T\colon \cZ\times 2^{[n]} \to \cZ$ a Tampering algorithm for $\cZ$ if $ \forall i \not\in s, z\in \Supp(Z), A(z,s)_i=z_i$.
\end{definition}





\begin{theorem} \cite{mahloujifar2017blockwise,mahloujifar2017learning} \label{thm:ptam}
For any product distribution $Z \equiv (Z_1 \times \dots \times Z_n)$ and any function $f\colon\Supp(Z) \to [0,1]$ where $\mu = \Ex_{z\gets Z}[f(Z)]$ and constant $0<p<1$ there is a tampering algorithm $T$ for $Z$ where
\begin{displaymath}
\Ex_{z\gets Z, s\gets S_{n,p}}[f(T(z,s))] \geq \mu + \frac{p}{1-p+p\cdot \mu} \cdot \Var_{z \gets Z}[f(z)]\,,
\end{displaymath}
where $S_{n,p}$ is the Binomial distribution over $n$ Bernoulli random variables with probability $p$. Moreover, if $Z_i$'s are efficiently samplable and $T$ is given oracle access to $f(\cdot)$, it could be implemented in polynomial time.
\end{theorem}




% \begin{corollary}
% For every $r \in [n]$ there is a tampering algorithm $T$ for $Z$ and a set $s\subset [n]$ of size $|s| \leq p\cdot n$ such that 
% $$\Ex[f(T(Z,s))] \geq \Ex[f(Z)] + p \cdot \Var[f(Z)] - \epsilon(n)$$
% \end{corollary}

\begin{corollary}\label{cor:biaslearn}
 Suppose $\problem=(\X,\Y,\D,\C,\hypoC,\loss)$ is a learning problem with bounded loss $\loss(h,x,y) \in [0,1]$, $\X$ is a product instance space $\X = \prod_{i \in [n]}\X_i$,  $\D$ contains product distributions $D_1\times\dots\times D_n$ over $\X_1,\dots,\X_n$, and $\BHD$ is the  Hamming distance over $\X$ (with $n$ blocks). If $\mu = \Risk(h,X,c), \nu=\Var_{x\gets X}[\loss(h,x,c(x))]$ for some $c \in \C, h\in \H$, then for all constants $p,\delta <1$ we have:
\begin{displaymath}
\Risk\eDR_{\BHD,(p+\delta) n}(h,X,c)\geq  \mu + \frac{p}{1-p+p\cdot \mu} \cdot\nu - \e^{-\frac{n\cdot \delta^2}{3p}}\,.
\end{displaymath} 
Moreover if $D_i$'s are efficiently samplable, and if we have oracle access to the function $f(x)=\loss(h,x,c(x))$, then the attack could be implemented in polynomial time.
\end{corollary}

\begin{proof}
Theorem \ref{thm:ptam} shows that if we sample $s$ from $S_{n,p}$ there is a tampering attack $T$ that can bias the average of loss function by $\frac{p}{1-p+p\cdot \mu}\cdot \nu$. The only issue is that the sampled set $s$ sometimes might have more than $(p+\delta)\cdot n$ blocks. However, using Chernoff bound we get
\begin{displaymath}
\Pr_{s\gets S_{n,p}}[|s| > (\delta+p)\cdot n] \leq \e^{-\delta^2\cdot n/(3\cdot p)}\,.
\end{displaymath}
Therefore, if we modify $T$ and abort anytime that $|s| > (\delta+p)\cdot n$, it only affects the average  of the adversarial DR risk by at most $\e^{-\delta^2\cdot n/(3\cdot p)}$ because the loss function is bounded to be at most $1$. Finally, using a basic averaging argument, we can always fix the randomness of $T$ and the randomness of selecting $s$ to a fixed value while still we achieve adversarial DR risk at least 
$\mu + \frac{p}{1-p+p\cdot \mu} \cdot\nu - \e^{-\frac{n\cdot \delta^2}{3p}}$.

The efficient variant of the attacker $T$ of Corollary \ref{cor:robustness} directly follows from the efficient variant of the biasing attack of Theorem \ref{thm:ptam}.
\end{proof}



==> ExactConstants.tex <==
\section{Finding Constants}

\Mnote{The following is Theorem 3 from \\ \url{https://people.maths.bris.ac.uk/~mb13434/Stirling_DeMoivre_Laplace.pdf}. Is there a version that bounds each side rather than bounding both sides?}
\begin{lemma}[Global form of the DeMoivre-Laplace Theorem]
Let $p\in(0,1)$ and $a<b$ be constants, and $X \equiv \Binom(n,p)$. Then
\begin{displaymath}
\lim_{n \to \infty} \Pr\left[a \leq \frac{X-np}{\sqrt{n\cdot p\cdot (1-p)}}  < b\right] = \Phi(b)-\Phi(a)\,.
\end{displaymath}

%Thus, for the special case of $a=-b$, the above probability becomes $$\sqrt{\frac{2}{\pi}} \int_0^{b} e^{-t^2} dt .$$
\end{lemma}

\paragraph{Notation.} Let $\ball(x,t)=\set{y \mid \HD(x,y) \leq t}$, and $B(n,t) = |\ball(x,t)|$ which is equal to $\sum_{k=0}^t \binom{n}{k}$ for all $x \in \bits^n$, and let $b(n,t)=B(n,t)/2^n$.

\subsection{Risk}
Suppose a hypothesis $h$ and concept $c$ lead to original risk $\mu=\Pr_{x \gets U_n}[h(x) \neq c(x)]$, and $h=b(n,t)$. By the isoperimetric inequality of Theorem \ref{thm:hq1}, by using $r=n-2t$ perturbations, we can increase the adversarial risk to $b(n,n-t)=1-b(n,t-1)>1-b(n,t)=1-\mu$. Also, by using $r=\floor{n/2}-t$ perturbations, we can increase the adversarial risk to $b(n,\floor{n/2})\geq 1/2$ \Snote{I think it should be ceiling}. 


\subsection{Robustness}

\paragraph{Notation.} Let $B(n,t) = \sum_{k=0}^t \binom{n}{k}$, $C(n,t)=\sum_{k=0}^t (t-k)\binom{n}{k}$, and $\gamma(m)={2^{2m-1}}/{\binom{2m}{m}}$.

\begin{lemma}[Lemma 3.8.2 from \cite{lovasz2003discrete}] \label{lem:BallVolUp} If $1\leq k \leq \floor{n/2}$, then $B(n,k-1) < \binom{n}{k} \cdot \gamma({\floor{{n}/{2}}})$. 
\end{lemma}
\begin{proof}
Case of $n=2m$ is Lemma 3.8.2 in \cite{lovasz2003discrete}. Case of $n=2m+1$ follows from the case for $n=2m$ and Pascal's equality. \Mnote{to be added.}
\end{proof}


\begin{lemma} 
$C(n,t) <  B(n,t) \cdot \gamma(\floor{n/2})$.
\end{lemma}

\begin{proof} We write the proof for $n=2m$, and the proof for $n=2m+1$ is similar.
\begin{align*}
C(n,t)=\sum_{k=0}^t (t-k)\binom{n}{k} 
&= \sum_{k=1}^{t} \sum_{i=0}^{k-1} \binom{n}{i} \\
\text{ (by Lemma \ref{lem:BallVolUp}) } &< \sum_{k=1}^{t} \binom{n}{k} \cdot \frac{2^{n-1}}{\binom{n}{n/2}} \\
& < B(n,t)\cdot \frac{2^{n-1}}{\binom{n}{n/2}}\,.\qedhere
\end{align*} 
\end{proof}

\begin{corollary} If $B(n,t)=\mu \cdot 2^{n}$ for $\mu=\Theta(1)$, then ${C(n,t)}/{2^n} = \mu \cdot \beta \cdot \sqrt{n}$ where $\beta \to \sqrt{\pi/8}<0.63$ for $n \to \infty$. Thus, if $\mu \approx 0.01$ and $n \to \infty$, $\sum_{k=0}^t {C(n,t)}/{2^n} < 0.0063 \sqrt{n}$.
\end{corollary}

==> HammingGraph.tex <==
\section{Hamming Graph}



\paragraph{Notation.} Here we define some basic notations. 
\begin{itemize}
    \item {\bf Metric:}  
    \begin{itemize}
        \item For a metric  $\metric$ over set $\X$:
\begin{itemize}
    \item For $x,y \in \X$, by $\metric(x,y)$ we denote the distance from $x$ to $y$ under $\metric$ (if $\metric$ is a quasi-metric, $\metric(x,y)$ could be different from $\metric(y,x)$).
    \item For $x \in \X$ and $\cS \se \X$, we let $\metric(x,\cS)=\inf_{y \in \cS} \metric(x,y)$.
\end{itemize}

\item We call a metric $\metric$ over $\cX$ an \emph{integer metric}, if $\metric(x,y)\in \set{0,1,\dots}=\N$. We call an integer metric a \emph{graph metric}, if there is a graph $G$ over vertices $\X$ such that $\metric(x,y)$ is the length of the shortest path from $x$ to $y$ in $G$. We call a graph-metric $\metric$ a \emph{Hamming metric} (or an $\ell_0$ metric) if $\cX=\cX_1\times \dots \times \cX_n$ and $G$ is connects $x=(x_1,\dots,x_n)$ to $y=(y_1,\dots,y_n)$ if they differ only in one coordinate.

Our focus in this work is on Hamming distance (and thus, Hamming metrics) but we will state some of our lemmas/claims in more general forms (or comment about such more general statements) for further study and broader interest. Our results that are stated for integer metrics extend to quasi-metrics as well. 
    \end{itemize}
    
\item {\bf Probability/measure:}

\begin{itemize}
    \item For a discrete probability distribution $D$ over set $\X$ and $\cS \se \X$, by $D(\cS)$ we denote the probability of $\cS$ under $D$. We use $D(\cA)= \Pr_D[\cA]$ to denote the probability of event $\cA \se \cX$ under $D$ and we drop $D$ to write $\Pr[\cA]$ when $D$ is clear from the context. We  also use $D$ to denote a \emph{random variable}  distributed according to $D$.
    \item When $D$ is a measure, we use a similar notation to the discreet case. Namely, we let $\Sigma_D \se \bits^\cX$ (or simply $\Sigma$ when $D$ is clear from the context) be the $\sigma$-algebra over which the probabilities are defined. Then, for every $\cA \in \Sigma$, we let $D(\cA)= \Pr_D[\cA]=\Pr[\cA]$ denote the probability of $\cA$ under $D$.
\end{itemize}


\end{itemize}



\begin{definition}
Let $\dist$ be a discrete distribution over a countable set $\X$, and let $\metric$ be a metric over $\X$. For any set $\cS \se\X$ and $b \in [n]$,  we define the adversarial risk for $b$  as
\begin{displaymath}
\Risk_b(\cS,D) = \Pr_{x\gets \dist}[\metric(x,\cS) \leq b]
\end{displaymath}
and for any such $\cS$ and $\alpha \in (0,1]$, we define the (generalized) robustness for $\alpha$ as
\begin{displaymath}
\Rob_{\alpha}(\cS,D) = \inf_{D(\cS') \geq \alpha} \left[D(\cS')\cdot\Ex_{x \gets \dist\mid \cS'}[\metric(x,\cS)]\right]\,.
\end{displaymath}
If $\dist$ is a measure (instead of a discrete distribution), then ... If $\dist$ is an integer metric.. (inf becomes min) \Mnote{to be added.}
\end{definition}

\begin{definition}[Continuous Hamming Ball]
The continuous Hamming ball with radius $r$ and weight $t$ is defined as follows
\begin{displaymath}
\HB_n(r,t) = \set{x\in [0,1]^n \colon \Exists 1 \leq i_1<\dots<i_{n-r} \leq n, \Forall j \in [n-r], x_{i_j} \geq t }\,.
\end{displaymath}
We use $|\HB_n(r,t)|$ to denote the volume of the ball in Lebesgue measure. Also we use $\thresh{r,\gamma,n}$ to denote the weighting $t$ that creates a Hamming ball with radius $r$ and volume $\gamma$, i.e.,  $|\HB_n(r,\thresh{r,\gamma,n})| = \gamma$. 
Whenever it is clear from the context, we might write $\HB(r,t),\thresh{r,\gamma}$.
\end{definition}

\Mnote{Please show how to derive the inequalities below from Hoeffding. also, should not be some squaring in the exponent?}\Snote{Yes it should quadratic.}
\begin{lemma}[Implied by Hoeffding Inequality] \label{lem:hamhoef} The following inequalities hold. 
\begin{itemize}
    \item $\Forall 0\leq r<t\cdot n, |\HB(r, t)|\leq e^{\frac{-2\cdot(t\cdot n - r)^2}{n}}$
    \item $\Forall t\cdot n< r\leq n, |\HB(r, t)|\geq 1 - e^{\frac{-2\cdot(r-t\cdot n)^2}{n}}.$
\end{itemize}
\end{lemma}




\begin{theorem}[Risk Lower Bound \textbf{CITATION MISSING}]
Let $\dist $ be the product Lebesgue measure over $[0,1]^n$. For any set $\cS\subseteq \R^n$ such that $\Pr_{x\gets \dist}[x\in \cS]=\gamma$ and $b\in[n]$ we have,
\begin{displaymath}
\Risk_b(\cS,D) \geq \min_{r\in[n-b]}\left|\HB(r+b,\thresh{r,\gamma})\right|\,.
\end{displaymath}
\end{theorem}


%\Mnote{I don't think the following is correct. You can have a measure over $R$ that does {\bf not} have a probability mass. I think each coordinate should be a real-valued random variable.See the wiki.\url{https://en.wikipedia.org/wiki/Random_variable#Real-valued_random_variables}}

\begin{corollary}\label{cor:main}
Let Let $\dist = (\dist_1 \times \dots \times \dist_n)$  where each $D_i$ is either a discrete or a real-valued random variable. For any set $\cS\subseteq \R^n$ such that $D(\cS)=\gamma$ and $b\in[n]$ we have,
\begin{displaymath}
\Risk_b(\cS,D) \geq \min_{r\in[n-b]}\left|\HB(r+b,\thresh{r,\gamma})\right|\,.
\end{displaymath}
\end{corollary}

\begin{proof}
Pending ....
\end{proof}



\begin{corollary}\label{cor:1to99}
Let $\dist = (\dist_1 \times \dots \times \dist_n)$  where each $D_i$ is a real-valued random variable.  For any $0\leq \gamma \leq \frac{1}{2} \leq 1- \gamma'\leq 1$ and any set $\cS\subseteq\R^n$ such that $D(\cS)=\gamma$ we have 
$\Risk_b(\cS,D) \geq 1- \gamma'$ for $b=\sqrt{\frac{-\ln(\gamma)\cdot n}{2}} + \sqrt{\frac{-\ln(\gamma')\cdot n}{2}}.$
\end{corollary}
\begin{proof}
By Hoeffding inequality we have 
\begin{displaymath}
\gamma = |\HB(r,\thresh{r,\gamma})| \leq e^{\frac{-2\cdot h^2}{n}} 
\end{displaymath}
where $h = \thresh{r,\gamma}\cdot n - r$. 
Therefore we have $h \leq \sqrt{\frac{-n\cdot\ln(\gamma)}{2}}$. 
On the other hand we have, 
\begin{displaymath}
|\HB(r+b, t(r,\gamma)| \geq |\HB(r+h+ \sqrt{\frac{-\ln(1-\gamma')\cdot n}{2}},\thresh{r,\gamma})| \geq 1 - e^{\ln(1-\gamma')}=\gamma'
\end{displaymath}
where the first inequality comes from the fact that $h \leq \sqrt{\frac{-n\cdot\ln(\gamma)}{2}}$ and $|\HB(r,t)|$ is an increasing function w.r.t $r$.  and the second inequality follows from the Hoeffding inequality. Therefore by applying Corollary \ref{cor:main} we have
$\Risk_b(\cS,D) \geq \gamma'$.
\end{proof}

\begin{corollary}\label{cor:1to99_limit}
Let $\dist = (\dist_1 \times \dots \times \dist_n)$  where each $D_i$ is a real-valued random variable and $n$ is sufficiently large.  For any $0\leq \gamma \leq \frac{1}{2} \leq 1- \gamma'\leq 1$ and any set $\cS\subseteq\R^n$ such that $D(\cS)=\gamma$ we have 
$\Risk_b(\cS,D) \geq 1- \gamma'$ for $b\approx \sqrt{n}\cdot(\Phi(1-\gamma')-\Phi(\gamma)).$
\end{corollary}

\begin{proof}
Let $r^*= \argmin_{r\in[n-b]}\left|\HB(r+b,\thresh{r,\gamma})\right|$ and $t^* = \thresh{r^*, \gamma}$. 
By Lemma \textbf{??} we have,
\begin{displaymath}
\gamma = |\HB(r^*,t^*)| \approx \Phi(\frac{r^* - n\cdot t^*}{\sqrt{n\cdot t^* \cdot(1-t^*)}})\,.
\end{displaymath}
Therefore, 
$r^* \approx n\cdot t^* + \Phi^{-1}(\gamma)\cdot \sqrt{t^*\cdot (1-t^*) \cdot n}$. Now by Corollary \ref{cor:main} we have
\begin{align*}
\Risk_b(\cS,D) &\geq|\HB(r^*+b, t^*)|\\
&\approx |\HB(n\cdot t^* + \Phi^{-1}(\gamma)\cdot \sqrt{t^*\cdot (1-t^*) \cdot n} - \frac{\Phi^{-1}(\gamma)}{2}\cdot \sqrt{ n} + \frac{\Phi^{-1}(1-\gamma')}{2}\cdot\sqrt{n} )|\\
&\geq |\HB(n\cdot t^* + \frac{\Phi^{-1}(1-\gamma')}{2}\cdot\sqrt{n})|\\
&\geq \Phi\left(\frac{\Phi^{-1}(1-\gamma')}{2\cdot\sqrt{t^*\cdot (1-t^*)}}\right)\\
&\geq \Phi\left(\Phi^{-1}\left(1-\gamma'\right)\right)\\
&= 1-\gamma'\,.\qedhere
\end{align*}
\end{proof}

\begin{definition}[Good Measure]
A measure space $D=(\X,A,D)$ is a good measure w.r.t a metric $M$ if
\begin{enumerate}
    \item $\Forall S\in A, \Forall h\in \R, \set{x\in X \colon \metric(x,\cS) = i} \in A$.
    \item there exist a function $f_D: A \times [0,1] \to A$, such that $\Forall S\in A, \Forall c\in [0,1], f_D(\cS,c)\subseteq \cS \wedge D\left(f_D(\cS,c)\right) = c\cdot D(\cS).$ 
\end{enumerate}
\end{definition}

\begin{lemma}\label{lem:risktorob-continuous}
for a metric space $(X,D)$ equipped with a good measure $D$ we have
\begin{displaymath}
\Rob_\alpha(\cS,D) = t\cdot \alpha - \int_{z=0}^{t} \Risk_i(\cS,D)\cdot dz
\end{displaymath}
where $t$ is the smallest number such that $\Risk_t(\cS,D) \geq \alpha$.
\end{lemma}

\begin{lemma} \label{lem:risktorob}
For a discrete metric $M$ that takes values in $\N$ and a \it{Good} Measure $D$ We have
\begin{displaymath}
\Rob_\alpha(\cS,D) = t\cdot \alpha - \sum_{i=1}^{t-1} \Risk_i(\cS,D)
\end{displaymath}
where $t$ is the smallest number such that $\Risk_t(\cS,D) \geq \alpha$. In particular, if every two points in $\X$ have distance at most $r$ (i.e., $r$ is bigger than or equal to  the diameter of $\X$), then 
\begin{displaymath}
\Rob(\cS,D)=\Rob_1(\cS,D) = r- \sum_{i=1}^r \Risk_i(\cS,D)\,.
\end{displaymath}
\end{lemma}
\begin{proof}
Let $\cS'\subseteq [0,1]^n$ be an arbitrary set such that $D(\cS')\geq \alpha $, \Mnote{that set might not exist. There might be a sequence converging to something.}\Snote{It exists for discrete distributions. For continuous distributions, it is sufficient to select a set that is very close to the infimum} \Mnote{So, first write the proof saying this is for discrete, and then write briefly at the end what parts need to change for the other case.} \Snote{Actually, I did not need to take the argmin.}
\remove{namely 
$$\cS' =  \argmin_{D(\cS') \geq \alpha} \left[D(\cS')\cdot\Ex_{x \gets \dist\mid \cS'}[\metric(x,\cS)]\right].$$
Since $D$ is a \it{Good} measure we have $D(\cS') = \alpha$ because if it is larger than $\alpha$ we can decrease its size without hurting the minimization.
}
For all $i\in [n]$ let $v_i = D(\set{x\in \X \colon \metric(x,\cS) = i}\cap \cS')$. We also define $v'_i$ as follows.
\begin{displaymath}
v'_i = \begin{cases} 
      \Risk_i(\cS,D) - \Risk_{i-1}(\cS,D) & 1\leq i\leq t-1 \\
      \alpha - \Risk_{t-1}(\cS,D) & i=t \\
      0 & i > t 
   \end{cases}
\end{displaymath}
Not that since $D$ is a good measure both $v'_i$ and $v_i$ are well defined. 
It is clear that $\sum_{i=1}^{n} v_i \geq \sum_{i=1}^{n} v'_i = \alpha$. We also have,
\begin{displaymath}
\Rob_\alpha(\cS,D) = \sum_{i=1}^{n} i\cdot v_i\,.
\end{displaymath}
It is also clear that
$\Forall i\leq t-1; v_i \leq v'_i$.
Now we prove that $\sum_{i=1}^{n} i\cdot v_i \geq \sum_{i=1}^{n} i\cdot v'_i$. 
\begin{align*}
    \sum_{i=1}^{t-1} i\cdot(v'_i - v_i) &\leq \sum_{i=1}^{t-1} t \cdot (v'_i - v_i)
    = t \cdot \sum_{i=1}^{t-1} (v'_i - v_i)
    \leq  t \cdot \sum_{i=t}^{n} (v_i - v'_i)
    \leq \sum_{i=t}^n i \cdot (v_i - v'_i).
\end{align*}

Therefore we have,
\begin{displaymath}
\sum_{i=1}^{n} i\cdot v_i \geq \sum_{i=1}^{n} i\cdot v'_i
\end{displaymath}
which implies 
$\Rob_\alpha(\cS,D) \geq \sum_{i=1}^{n} i\cdot v'_i$
On the other hand, we know that 
$\Rob_\alpha(\cS,D) \leq \sum_{i=1}^{n} i\cdot v'_i$ (because the robustness is minimized over all possible $v_i$'s).
Therefore,
\begin{align*}
    \Rob_\alpha(\cS,D) &= \sum_{i=1}^{n} i\cdot v'_i \\
    &= v'_t\cdot t + \sum_{i=1}^{t-1} i\cdot (\Risk_i(\cS,D) - \Risk_{i-1}(\cS,D)) \\
    &=   v'_t \cdot t + \Risk_{t-1}(\cS,D) \cdot (t-1) - \sum_{i=0}^{t-2}\Risk_i(\cS,D)\\
    &= t\cdot(v'_t + \Risk_{t-1}(\cS,D)) - \sum_{i=0}^{t-1} \Risk_i(\cS,D)\\
    &= t\cdot \alpha -  \sum_{i=0}^{t-1} \Risk_i(\cS,D)\,.\qedhere
\end{align*}
\end{proof}





\begin{theorem}[Robustness Upper bound]
Let $\dist = (\dist_1\times \dots \times  \dist_n)$ where each $D_i$ is a real-valued random variable. For any set $\cS\subseteq \R^n$ such that $D(\cS)=\gamma$ and $\alpha\in[\gamma,1]$ we have,
\begin{displaymath}
\Rob_{\alpha}(\cS,D) \leq (c_1\cdot\sqrt{-\ln(\gamma)}+c_2 +\alpha\cdot c_3)\cdot\sqrt{n}\,.
\end{displaymath}
\end{theorem}

\begin{claim}[\cite{kaas1980mean}] \label{cl:hb-half}
$|\HB(\ceil{t\cdot n}, t)| \geq 0.5~.$
\end{claim}

\begin{lemma}
We have
$\Rob_{0.5}(\cS,D) \leq  \sqrt{\frac{-\ln(\gamma)\cdot n}{8}}$
\end{lemma}
\begin{proof}
Let $b=\sqrt{\frac{-\ln(\gamma)\cdot n}{2}}$ by Theorem \ref{cor:main} we have,
\begin{displaymath}
\Risk_b(\cS,D) \geq \min_{r\in[n-b]}\left|\HB(r+b,\thresh{r,\gamma})\right|\,.
\end{displaymath}
Therefore there exist some $r^*\in [n]$ such that 
\begin{displaymath}
\Risk_b(\cS,D) \geq \left|\HB(r^*+b,\thresh{r^*,\gamma})\right|\,.
\end{displaymath}
Now let $h=n\cdot \thresh{r^*,\gamma}\cdot n - r^*$. By Hoeffding inequality we have $\gamma \leq e^{\frac{-2\cdot h^2}{n}}$ which implies $h \leq \sqrt{\frac{-\ln(\gamma)\cdot n}{2}}$. Therefore we have
\begin{displaymath}
\Risk_b(\cS,D) \geq \left|\HB(r^*+b,\thresh{r^*,\gamma})\right| \geq \left|\HB(r^*+h,\thresh{r^*,\gamma})\right| = \left|\HB(\thresh{r^*,\gamma}\cdot n,\thresh{r^*,\gamma})\right| \geq 0.5\,.
\end{displaymath}
where the last inequality follows from Claim \ref{cl:hb-half}. 
Now by Lemma \ref{lem:risktorob} we have,
\begin{displaymath}
\Rob_{0.5}(\cS,D) = 0.5\cdot t - \sum_{i=0}^{t-1} \Risk_i(\cS,D)  \leq 0.5\cdot t \leq 0.5\cdot h \leq 0.5\cdot b \,.\qedhere
\end{displaymath}
\end{proof}

\begin{lemma}
If $\alpha \geq |S| \geq 0.5$ then 
$\Rob_{\alpha}(\cS,D) \leq c_2 \cdot \sqrt{-\ln(\alpha)\cdot n}$
\end{lemma}

\begin{proof}
Let $t$ be the smallest number such that $\Risk_t(\cS,D) \geq \alpha$. 
By Theorem \textbf{??} we know that there exist $r^*\in [n] $ such that
$\Risk_{t-1}(\cS,D) \geq |\HB(r^* + t -1, \thresh{\gamma, r^*}|$. Therefore we have
$|\HB(r^* + t -1, \thresh{\gamma, r^*}| \leq \alpha$ which implies $t\leq \sqrt{\frac{-n\cdot\ln(1-\alpha)}{2}}+1$ by Hoeffding inequality. 
By Lemma \ref{lem:risktorob} we have,
\begin{align*}
\Rob_{\alpha}(\cS,D) &= \alpha \cdot t - \sum_{i=1}^{t-1} \Risk_i(\cS,D)
\end{align*}
By Theorem \textbf{??}we know that for each $i\in [t]$ there exist $r_i\in[n]$ 
such that $\Risk_i(\cS,D) \geq \HB(r_i +i , \thresh{\gamma, r_i})$. 
Note that we have $\gamma = |\HB(r_i, \thresh{\gamma, r_i}|\geq 0.5$ 
which implies $r_i \geq \floor{n\cdot \thresh{\gamma, r_i}}$ by Claim \ref{cl:hb-half}. Therefore,
\begin{align*}
\Rob_{\alpha}(\cS,D) &= \alpha \cdot t - \sum_{i=1}^{t-1} \Risk_i(\cS,D)\\
\text{(By Theorem \textbf{??})~~}&\leq \alpha \cdot t - \Risk_0(\cS,D) - \Risk_1(\cS,D) - \sum_{i=2}^{t-1} |\HB(r_i+i, \thresh{r_i,\gamma})|\\
\text{(By $\Risk_i(\cS,D) \geq 0.5$)~~}&\leq \alpha \cdot t - 1 - \sum_{i=2}^{t-1} |\HB(r_i+i, \thresh{r_i,\gamma})|\\
\text{(By Claim \ref{cl:hb-half})~~}&\leq \alpha \cdot t - 1 -\sum_{i=2}^{t-1} |\HB(\floor{\thresh{r_i,\gamma}\cdot n} + i, \thresh{r_i,\gamma})|\\
&\leq \alpha \cdot t - 1 -\sum_{i=2}^{t-1} |\HB(\thresh{r_i,\gamma}\cdot n + i -1, \thresh{r_i,\gamma})|\\
\text{(By Hoeffding Inequality)~~}&\leq \alpha \cdot t -1 -\sum_{i=2}^{t-1} (1-e^{\frac{-2(i-1)^2}{n}})\\
&\leq \alpha \cdot t  -t + 1   + \sum_{i=2}^{t-1} e^{\frac{-2(i-1)^2}{n}}\\
&\leq 1   + \sum_{i=2}^{t-1} e^{\frac{-2(i-1)^2}{n}}\\
& \leq 1 + \int_{0}^{t-2} e^{\frac{-2x^2}{n}}dx\\
&=  1 + \frac{\sqrt{n\pi}}{2} \cdot \erf(\frac{t-2}{\sqrt{n}})\\
&\leq  1 + \frac{\sqrt{n\pi}}{2} \cdot \erf(\sqrt{\frac{-\ln(1-\alpha)}{2}})\\
&\leq \frac{\sqrt{n\cdot \pi}}{2} \cdot(1- \sqrt{\frac{e}{2\pi}}\cdot(1-\alpha))\,.\qedhere
\end{align*}
\end{proof}


==> approxEntropy.tex <==
\subsection{Approximating Solutions of the Entropy Function}
\begin{lemma}\label{lem:entropy:upper_bound:key}
Let $p\in(0, 1/2]$. Then, $-(1-p)\lg(1-p) \le p\lg(3)$.
%Let $p\in(0, 1/2]$. Then, $-(1-p)\lg(1-p) \le 2p$.
\end{lemma}
\begin{proof}
Let $f(p) = p\lg(3) + \lg(1-p) - p\lg(1-p)$ with $p\in[0, 1/2]$.
The derivative is
$f'(p) = \frac{\ln 3}{\ln 2} - \frac{1}{(1-p)\ln 2} - \frac{\ln (1-p)}{\ln 2} + \frac{p}{(1-p)\ln 2}
= \frac{1}{\ln 2}\cdot(-1 + \ln 3 - \ln(1-p))$.
We have $f'(p) \ge 0 \Rightarrow \ln(1-p) \le \ln(3/e) 
\Rightarrow 1 - p \le 3/e \Rightarrow p \ge 1 - 3/e \approx -0.1$,
which is true.
Therefore, 
for every $p\in(0, 1/2]$, we have 
$f(p) \ge \lim_{p\rightarrow 0^+} f(p) = 0$.
In other words, the statement holds.
%
%Let $f(p) = 2p + \lg(1-p) - p\lg(1-p)$ with $p\in[0, 1/2]$.
%The derivative is
%$f'(p) = 2 - \frac{1}{(1-p)\ln 2} - \frac{\ln (1-p)}{\ln 2} + \frac{p}{(1-p)\ln 2}
%= \frac{1}{\ln 2}\cdot(-1 + 2\ln 2 - \ln(1-p))$.
\end{proof}

\begin{lemma}\label{lem:entropy:lower_bound:key}
Let $p\in\left(0,\frac{e-2}{e}\right]$. Then, 
$-(1-p)\lg(1-p) \ge p\lg(2)$.
\end{lemma}
\begin{proof}
Let $f(p) = -(1-p)\ln(1-p) - p\ln(2)$.
Then, $f'(p) = (p\ln(1-p) - \ln(1-p))' - \ln(2) 
= \ln(1-p) - \frac{p}{1-p} + \frac{1}{1-p} - \ln(2)
= \ln(1-p) + 1 - \ln(2) = \ln(1-p) - \ln(2/e)$.
Therefore, $f'(p) \ge 0 \Rightarrow p \le 1 - 2/e$.
In other words, $f$ is increasing for every $p\in(0, 1-2/e]$
and hence $f(p) \ge \lim_{p\rightarrow 0^+} f(p) = 0$.
\end{proof}

\begin{lemma}\label{lem:entropy:general_lower_bound:key}
Let $f(p) = -p(\lg(3/p))^2$ with $p\in(0, 1/2]$.
Then, $f(p) > -4$.
\end{lemma}
\begin{proof}
The derivative of $f$ is,
$f'(p) = \frac{-(\ln(3/p))^2 + 2\ln 3 + 2\ln(1/p)}{(\ln 2)^2}$.
Therefore we have $f'(p) \ge 0 \Rightarrow
-(\ln 3)^2 - 2(\ln 3)\ln(1/p) - (\ln(1/p))^2 + 2\ln 3 + 2\ln(1/p) \ge 0
\Leftrightarrow
-y^2 + 2(1-\ln 3)y - (\ln 3)(\ln 3 - 2) \ge 0$
for $y = \ln(1/p)$.
The quadratic has discriminant $4$ and the two solutions are
$y_1 = -\ln 3$ and $y_2 = 2 - \ln 3$.
But then this means that $f$ increases when $\frac{3}{e^2} \le p \le 3$
and decreases otherwise. 
Therefore, the minimum value of $f$ is obtained at $p = 3e^{-2} \approx 0.406$,
in which case we have $f(3e^{-2}) = -\frac{12}{e^2(\ln 2)^2} \approx -3.38 > -4$.
\end{proof}

\begin{lemma}\label{lem:entropy:bound_general_solution}
Let $0 < c < 1$ and $0 < p \le 1/2$.
Then, $H(p) = c \Rightarrow
\frac{c}{2\lg(4/c)} < p < \frac{c}{\lg(1/c)}$.
\end{lemma}
\begin{proof}
Using Lemma \ref{lem:entropy:upper_bound:key} we observe that, 
\begin{displaymath}
p\lg(1/p) < H(p) = -p\lg(p) - (1-p)\lg(1-p) \le -p\lg(p) + p\lg(3) = p\lg(3/p)\,.
\end{displaymath}
We have $H(p) = c$.
Since $p\lg(1/p) < c = H(p)$ we have that $p < c$.
But then $1/p > 1/c$ and further $\lg(1/p) > \lg(1/c)$.
So, we have that $p\lg(1/p) < c \Rightarrow p < \frac{c}{\lg(1/p)} < \frac{c}{\lg(1/c)}$.

On the other hand, 
$c \le p\lg(3/p)$.
Let $c \le x = p\lg(3/p)$. Then, $c^2 \le x^2 < \frac{16}{3}p$.
To see this, note that we require, 
$x^2 = p^2(\lg(3/p))^2 < \frac{16}{3}p
\Leftrightarrow 
p(\lg(3/p))^2 < 16/3$.
But this is true due to Lemma \ref{lem:entropy:general_lower_bound:key}.
In other words it holds, $3c^2 < 16p \Leftrightarrow \frac{3}{p} < \left(\frac{4}{c}\right)^2
\Leftrightarrow \lg(3/p) < 2\lg(4/c)$.
So, starting again from $c\le  p\lg(3/p)$, we have that 
$p \ge \frac{c}{\lg(3/p)}$ and due to the last observation we have $p > \frac{c}{2\lg(4/c)}$.

Finally, note that the upper bound is very loose for $c > 1/2$, since we have a
trivial upper bound for $p$ being at most $1/2$ for any $1/2 < c \le 1$.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Better bound for restricted p
%
%\begin{comment}
\begin{lemma}
%Let $e \approx 2.71828...$
Let $0 < c \le 0.833 < H\left(\frac{e-2}{e}\right)$.
Let $0 < p < (e-2)/e \approx 0.26424$.
Then $H(p) = c$ 
%\Rightarrow 
implies that 
$p\in\left[\frac{c}{2\lg(4/c)}, \frac{c}{\lg(5.84/c)}\right] $
%\subseteq \left[c^2/8, c/2.8\right]$. %\frac{c^2}{8}, \frac{c}{3}\right]$
%\Rightarrow p\in\left[\frac{c}{2\lg\frac{4}{c}}, \frac{c}{\lg\frac{6}{c}}\right] 
%\subseteq \left[\frac{c^2}{8}, \frac{c}{3}\right]$
\end{lemma}
\begin{proof}
The lower bound for the solution $p$ is obtained as in Lemma \ref{lem:entropy:bound_general_solution}
starting from the inequality $c \le p\lg(3/p)$.

For the upper bound for the solution $p$ this time 
we exploit the fact that $c < H\left(\frac{e-2}{e}\right)$.
Due to Lemma \ref{lem:entropy:lower_bound:key} we have that
$H(p) = -p\lg(p) - (1-p)\lg(1-p) \ge p\lg(1/p) + p\lg(2) = p\lg(2/p)$.
But then, $p\lg(2/p) \le c = H(p)$. The first observation is that 
$p \le \frac{c}{\lg(2/p)} \le \frac{c}{\lg\left(\frac{2e}{e-2}\right)} < \frac{c}{2.92}$.
But then this means that
$p \le \frac{c}{\lg(2/p)} \Rightarrow p \le \frac{c}{\lg\left(\frac{5.84}{c}\right)}$.
%On the other hand, $p\le \frac{c}{\lg(2/p)} \le \frac{c}{\lg\left(\frac{2e}{e-2}\right)}$
\end{proof}
%\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> attacks.tex <==
\section{Attacks}

%\input{AttacksGeneric.tex}

\input{AttacksSpecific.tex}

==> generalProblems.tex <==
\section{Two General Problems}
In this section we describe two general problems. 
Let $M$ be a metric over $\X$
and let $\dist$ be a distribution over \X. 
Let $R\subseteq \X$. 
Denote $\norm{R}_{\dist} = \probsub{x\from\dist}{x\in R}$.
Further let, 
$B_{r}(x) = \set{x' | M(x, x') \le r}$, 
$B_{r}(R) = \cup_{x\in R} B_{r}(x)$ and 
$G_R(x) = \min_{x'\in R} M(x, x')$.
Then, we would like to solve the two problems shown below.
\begin{eqnarray}
\min_{R} & \norm{B_{r}(R)}_{\dist} \label{problem:mvg} \\
\max_{R} & \expectedsub{x \gets \dist}{G_R(x)} \label{problem:med}
\end{eqnarray}
We call a solution $R$ to (\ref{problem:mvg}) a solution to the \emph{minimum volume growth} problem,
whereas a solution $R$ to (\ref{problem:med}) a solution to the \emph{maximum expected distance} problem.

%\paragraph{The Minimum Volume Growth Problem.} 
%\begin{displaymath}
%\min_{R} \norm{B_{r}(R)}_{\dist}
%\end{displaymath}


%\paragraph{The Maximum Expected Distance Problem.}
%We want, 
%\begin{displaymath}
%\max_{R} \expectedsub{x \gets \dist}{G_R(x)}
%\end{displaymath}



==> intro_Backup.tex <==
\section{Introduction}
In recent years, neural networks have pushed to new heights
the classification results on traditional datasets 
that are used as testbeds for various machine learning methods\footnote{For example,
a summary of state-of-the-art results is available at 
\href{http://rodrigob.github.io/are_we_there_yet/build/}{http://rodrigob.github.io/are\_we\_there\_yet/build/} .}. 
As a result, the properties of the various classification methods have been put further into scrutiny.
%In particular, one such direction of adversarial machine learning deals
In particular, studying the robustness of the trained models under malicious attacks have gained increased popularity.

Within adversarial machine learning, 
one such 
direction of research 
that has gained popularity in recent years  
deals with 
%what is 
the study of the 
%studies the 
so-called \emph{adversarial perturbations} of the test instances.
%In the context of deep learning classifiers %was 
This line of work was  particularly
popularized, in part, by the work of \citep{Szegedy:intriguing}
 within the context of deep learning classifiers.
%but there is lots of related work; e.g., \citep{Adversarial::Harnessing,DeepFool,CarliniWagner} to name a few.
%
Briefly, %adversarial perturbations 
when one is given a particular instance for classification, 
an adversarial perturbation for that instance is a (minimal) change on the features of the instance so that when this change is added to the instance, the resulting perturbed instance is misclassified. 
The resulting perturbed instance is commonly referred to as an \emph{adversarial example}. 
The work of \citep{Szegedy:intriguing} revealed pairs of images that 
%could be obtained 
%by adding a small distortion (perturbation) to other images, 
differed slightly 
so that a human eye could not
identify any real differences between the two, % images 
and yet, 
contrary to what one would naturally expect, 
machine learning classifiers would predict different labels for the classifications of such pairs of images.
%therefore one would naturally expect from a machine learning classifier to predict the same class for both 
%of the images, which turned out not to be true in practice.
%
Within this context, a very intense line of work started, aiming to understand and explain 
the properties of machine learning classifiers and such adversarial perturbations; e.g., \citep{Adversarial::Harnessing,DeepFool,Adversarial::Constraints,CarliniWagner,madry2017towards}. These attacks are sometimes referred to as \emph{evasion} attacks \cite{nelson2012query,biggio2014security,Adversarial::Harnessing,CarliniWagner,Adversarial::FeatureSqueezing}.

%would thus one reasonably expect that a classifier would predict the same classification for both images
%certainly the expectation in such a setting
%classification of the two 
We note that there is indeed earlier work in this framework;
e.g., \citep{Adversarial:Old,Adversarial:models},
and generally speaking, 
it is no big surprise that when one has not learned the ground truth precisely, there can be pairs of instances 
that are almost similar under some metric, but one of them is misclassified. 
%that are classified differently 
However, it is perhaps the striking resemblance to the human eye 
of the pairs of images that were provided in \citep{Szegedy:intriguing}
that really gave this new push for intense investigations within the context 
of adversarial perturbations and related notions.
%
%The current paper continues the study of adversarial perturbations.
%
%In multi-class classification,  the study of adversarial perturbations  can be further refined to \emph{untargeted} and \emph{targeted} attacks. For targeted attacks one not only wants to compute a change that when added to an instance gives rise to a misclassified instance (which is what plain untargeted attacks aim for), but also, one has a particular target class in mind and the goal is to cause the classifier to predict that the perturbed instance belongs to that particular class (and this is a mistake).
%
%Note that 

There are other directions of research under the umbrella of adversarial machine learning, 
such as designing defenses against adversarial examples as in \citep{Defenses:Distillation,Adversarial::FeatureSqueezing}, 
or poisoning (aka causative) attacks that aim to ruin the accuracy of classifiers by being able to tamper with 
part of the training process as in \citep{awasthi2014power,xiao2015feature,shen2016uror,mahloujifar2017learning}. 
Our focus in this work is to do a formal study of the power of adversarial perturbations of the input instances.

\subsection{Our Approach and Results}
Previous studies of adversarial perturbations use different ``definitions of security'' to model the adversary's goal. Our contribution in this work is twofold: 
(1) developing a taxonomy for various ways of formalizing  the risk and robustness under adversarial perturbations, and 
(2) studying generic attacks that apply to a broad class of learning problems and (3) studying  attacks for the specific case of monotone conjunctions under tampering with test inputs that are drawn from the uniform distribution. 
Our specific study of the problem of monotone conjunctions shows that previous definitions of
the adversarial risk and robustness lead to different bounds compared to actually asking the adversary to push the instances into the disagreement region of the trained hypothesis and the actual ground truth (i.e. the target concept). Thus, a direct definition of adversarial risk and robustness seems necessary for a broader study in this field.

\subsubsection{Defining Adversarial Risk and Robustness}

Here we  briefly explain the core ideas behind some previous definitions and how they compare with our new definitions. 
For simplicity we focus on the %simpler 
case of \emph{classification} problems where $c(x)$ is the correct label for an instance $x\in\X$.  
The adversary aims to perturb the instance $x$ into an instance $x'$ such that 
$x'$ is close to $x$ under some metric and moreover 
$x'$ is misclassified by the trained hypothesis $h$. By \emph{risk} we refer to the probability by which the adversary can get a misclassified $x'$ `close' to $x$, and by \emph{robustness} we refer to the minimum change to $x$ that can guarantee $x'$ is misclassified.

\emph{Risk and robustness based on the original prediction.} 
%\paragraph{Risk and Robustness Based on the Original Prediction.} 
The work of  \citep{Szegedy:intriguing} %\cite{madry2017towards} 
modeled adversary's job as perturbing the instance $x$ into the close instance $x'$ such that $h(x')\neq h(x)$.\footnote{\citep{Szegedy:intriguing} focuses on the $||\cdot ||_2$ norm, and also studies the \emph{targeted} perturbations where the adversary has  a specific target label in mind.}  
(See Definition \ref{def:PC} for a formalization.) 
Note that, $x'$ would indeed be a misclassification if $c(x') \neq h(x)$, but by substituting this condition with $h(x')\neq h(x)$ one can use optimization methods to find such a close point $x'$ solely based on the parameters of the trained model $h$. 
However, this approach is based on two implicit assumptions: (1) that the  hypothesis $h$ is  correct on all the original untampered %test 
examples $x \gets \dist$; we call this the \emph{initial correctness} assumption, and that (2) the ground truth $c(\cdot)$ does not change under small perturbations of $x$ into $x'$ (i.e., $c(x) = c(x')$); we call this the \emph{truth proximity} assumption. 
However, if either of these to implicit  assumptions do not hold, we cannot use the condition $h(x')\neq h(x)$ as adversary's goal in formalizing the the adversarial risk and robustness.
We refer to this approach as the \emph{prediction-change} (PC) approach.



\emph{Risk based on the original label.}
%\paragraph{Risk Based on the Original Label.} 
The recent work of %Madry et al. 
\citep{madry2017towards} proposed a new way of defining an adversarial loss and risk based on adversary's ability to obtain an $x'$ close to $x$ such that $c(x) \neq h(x')$; 
namely, here we compare the new prediction to the old actual label (see Definition \ref{def:OL}). 
This definition %, now 
has the advantage that it no longer relies on the implicit assumption of initial correctness for $x \gets D$. 
However, %in order for 
$x'$ is misclassified %in the disagreement region, 
%we still need to make 
only under 
the truth proximity assumption; that is, one still needs to assume $c(x') = c(x)$.
We refer to this approach for defining adversarial risk and robustness as the \emph{old-label} (OL) approach.

%Indeed, if $x'$ is close enough to $x$ (i.e., $x' \in M_r(x)$ for sufficiently small $r$) it will likely imply that the true labels of $c(x),c(x')$ are the same, and so it  would indeed hold that $h(x') \neq c(x)=c(x')$ meaning $x'$ is classified by $h$. However, we emphasize that here there is an implicit assumption on $c(x)=c(x')$. For natural scenarios like classification of images under adversarial noise (see \Mnote{need to cite here?}) this implicit assumption is likely to hold: small perturbations  do not change the classification in humans' eyes. More formally, we say that the \emph{truth proximity} assumption holds over the  set $\cI \subseteq \X$ of test examples, the concept $c(\cdot)$ and the metric $M$ over the input instances as well as the threshold $r$, if for all $x \in \cI$ and all $x' \in M_r(x)$ we have that $c(x) = c(x')$.

%\Dnote{There is something wrong in the above definition. With original label we want $c(x) \neq c(x')$. It is true that the MIT version is looking at $h(x') \neq c(x)$ and I believe they use the truth proximity assumption, which is why we want to end up discussing $h(x') \neq c(x') = c(x)$ in their context. But this is not original label.}



%\paragraph{Our Approach: Working with the Disagreement Region.}
%\paragraph{Our Approach: Disagreement Region.}
%{\bf Our approach: directly working with the disagreement region.} 
{\bf Our approach: disagreement region.}
In this work, we propose  defining adversarial risk and robustness  (see Definition \ref{def:DR})  directly based on requiring the adversary to push the instances into the disagreement region \emph{regardless} of whether or not %either of
the truth proximity or the initial correctness assumptions hold.
Namely, our adversary simply aims to perturb $x$ into a close $x'$ such that $h(x') \neq c(x')$. 
The main
motivation for %our revisited formalization of 
revisiting 
these notions,  
is that in broader settings where either of the truth proximity or the initial correctness assumptions do not hold, 
our new definitions of adversarial risk and robustness are still meaningful 
while the previous definitions 
%(based on the original label and prediction) 
no longer guarantee misclassification of $x'$. 
%We further give a stronger definition of risk and robustness that requires the stronger condition for the perturbed $x'$ that $c(x)=c(x')\neq h(x')$. Any attack under such condition would be s
We % refer to this approach as 
call this the 
\emph{disagreement-region} (DR) approach.

\subsubsection{Generic Attacks}
We show that when one defines the risk and robustness directly based on the disagreement region, then there are nontrivial attacks in cryptographic contexts and analysis of bounded functions that lead to lower bounds on the adversarial risk and robustness under the \emph{uniform} product distribution.

\emph{Information theoretic attacks.} In particular, we show that the biasing attack of \cite{lichtenstein1989some} against the security of adaptive coin tossing protocols imply that the adversarial robustness of \emph{any} classification problem under the uniform distribution $U_n$ of dimension $n$ is upper bounded by $\approx \sqrt{n \log (1/\mu)}$ where $\mu$ is the original risk without the attack. This shows that for constant original risk $\mu$, the amount of perturbation necessary to misclassify $x$ is \emph{sub-linear} in the dimension $n$. This attack, however, is information theoretic, and only shows the \emph{existence} of such adversarial misclassified input $x'$.

\emph{Computationally bounded attacks.} We further show that the recent, so called $p$-tampering attacks, of \cite{mahloujifar2017blockwise,mahloujifar2017learning} can also be applied to obtain generic attacks on the \emph{risk} of classification problems (or even problems with \emph{bounded} loss in $[0,1]$) when the input is uniform (or even comes from a product distribution). We show that such attacks can increase the risk, using the adversarial perturbed inputs, by $\Omega(p) \cdot c$ where $c$ is a constant that depends on the original risk without the perturbation, while the adversary only changes $p$ coordinates of the instance $x$. The main advantage of the $p$-tampering attacks is that they could run in \emph{polynomial time} if $h,c$ are efficiently computable.

\subsubsection{Attacking Monotone Conjunctions under the Uniform Distribution}
In addition to our generic bounds that we obtain using tools from cryptographic attacks, 
we also make a comprehensive study of a particular class of %hypothesis 
functions, namely the monotone conjunctions. %, under the uniform distribution. 
%The class of monotone conjunctions is PAC learnable and 
This class of functions is perhaps one of the most natural and basic examples 
studied in computational learning theory. 
For example, studying the learnability of monotone conjunctions under the uniform distribution was given as 
a paradigmatic example by Valiant when he introduced evolvability in \citep{Valiant::Evolvability},
which is a special form of PAC learning \citep{Valiant:PAC}.
%fundamental problems in computational learning theory
%In addition to being a natural fundamental problem studied already by Valiant and shown to be PAC learnable \citep{Valiant:PAC}, 
We %study this class of functions and 
attack such hypotheses under the uniform distribution 
in order to further demonstrate the different behavior of adversarial risk and robustness under various previous definitions and show that they do \emph{not} equate the right bounds provided by 
our DR approach.
%directly defining adversarial risk and robustness based on DR. %the disagreement region.



First of all, % \Mnote{adding the (DR) (PC) and (OL) to the above discussions}
our DR approach 
implies different results compared to 
the %prediction-change-based 
PC %approach
and the %old-label-based (OL) 
OL  
approach when $h = c$;
that is, when the ground truth has been identified completely.
%that is, when the learner has identified the ground truth precisely.
\if 0
For example, the risk in the DR approach is always $0$ no matter how many coordinates
the adversary can change on any given input $x$, % truth assignment, 
whereas the other two methods 
%allow positive risk and in fact 
allow 
the risk to be as large as 1 %for sufficiently high budget.
with sufficient budget.
\fi
However, there are differences even when $h \neq c$.
The robustness to adversarial perturbations
is 
$\Theta\left(\min\{\abs{h}, \abs{c}\}\right)$ 
in the %disagreement-region-based 
DR approach, %we obtain 
where $\abs{h}$ and $\abs{c}$ is the number of variables that appear in $h$ and $c$ respectively, 
whereas the %prediction-change-based 
PC %approach as well as the %old-label-based 
and 
OL approaches both imply robustness of $\Theta\left(\abs{h}\right)$.
As such, the values are wildly different when $h$ has many more variables compared to $c$.
%Similar differences can be identified for risk.
%For example, 
Regarding risk, %one example is the following scenario:
here is an example:
%consider the scenario where 
$h$ is a hypothesis that shares %$m = 100$ 
$m$
variables with the target $c$
and moreover $h$ 
has %$w = 50$ 
$w=m/2$
additional variables, %(that are wrong since they do not appear in $c$),
while $c$ has, apart from the %$m=100$ 
$m$
variables, 
%$u=10$ 
$u=m/20$
more variables that do not appear in $h$.
Then, %for example, 
%when one has 
with 
a budget of %size 
%$r = 55$,
$r=0.55m$
the DR approach indicates that the adversarial risk is at least $1/8$,
whereas the PC and the OL approaches predict risk less than 
$2^{-(1-H(0.55m/\abs{h}))\cdot \abs{h}}$,
where $H(\alpha)$ is the binary entropy of $\alpha$
and $\abs{h} = m + w = 3m/2$.

%\Dnote{I will add two more examples here with risk in the morning.
%One idea is DR vs PC: use upper bound based on entropy and show that with a certain budget
%our DR based approach allows the risk to be driven up to 1, whereas the PC based approach,
%by the `entropy' upper bound allows the risk to be as high as, say, $2^{-0.9n}$
%and thus there is a huge gap.
%Then, we have to think about a simple example with a gap between DR and OL.
%Ok, more tomorrow.}




\if 0
For example this is a common scenario when someone has learned monotone conjunctions
using the basic PAC learning algorithm by Valiant \citep{Valiant:PAC} that only looks at the positive examples, 
as the learned conjunctions contain all the variables that appear in the target
plus potentially lots of redundant variables.
In fact this very nature of the `vanilla' algorithm has an improved version
where set covering is used in order to exploit the negative examples as well and thus
reduce the number of redundant variables in the learned hypothesis. 
%Therefore, $\min\{\abs{h}, \abs{c}\}$ and $\abs{h}$ can be wildly different.
\fi

\if 0
{\centering
\begin{tabular}{c|c|c|c|}\cline{2-4}
               & DR & PC & OL \\\hline
\multicolumn{1}{|c|}{robustness} & $\Theta\left(\min\{\abs{h}, \abs{c}\}\right)$ & $\Theta(\abs{h})$ & $\Theta(\abs{h})$ \\\hline
\end{tabular}
}
\fi




==> prelim.tex <==
\section{Preliminaries}\label{sec:prelims}
\begin{definition}[Levy family]
A family $\set{(X_i, \metric_i, \mu_i}_{i\in\N}$ where $(X_i,\metric_i)$ is a metric space equipped with borel \Mnote{Borel!} measure $\mu_i$ is called a normal Levy family if there exist constants $c_1,c_2\in \R$ such that for all open sets $A\subset X$ such that $\mu(A)\geq \frac{1}{2}$ we have,
\begin{displaymath}
\mu(A_\epsilon) \geq 1 - c_1\cdot \exp(-c_2\cdot \epsilon^2 \cdot n)\,.
\end{displaymath}
\end{definition}






















%
%For any distribution $\dist$ over $\X \times \Y$, by $D_\X$ and $D_\Y$ we refer to the marginal distributions of the  components of $D$, and we let $(D_\X \mid y) \equiv (D_\X \mid D_\Y=y)$ and $(D_\Y \mid x) \equiv (D_\Y \mid D_\X=x)$ denote the conditional marginal distributions.
%



\if 0
%We use the terms \emph{generalization} and \emph{specialization} as in 
%Mitchell's framework of \emph{version spaces} 
%\citep{Mitchell::VersionSpaces}. %,Book::Mitchell:MachineLearning}.
%That is, %we say that 
We say that 
a Boolean function 
%$\upvarphi$ 
$f$ 
is a \emph{generalization} (resp., \emph{specialization}) 
of a Boolean function $f'$ iff
the set of satisfying truth assignments for $f$ 
is a \emph{superset} (resp., \emph{subset}) 
of the set of satisfying truth assignments for $f'$;
see \citep{Mitchell::VersionSpaces}.
We denote this relationship as $f \ge_g f'$ (resp., $f \le_g f'$).
When the set inclusion is strict 
%we say 
%\emph{strict generalization} (resp., \emph{strict specialization})
%and denote the relationship as 
we write 
$f >_g f'$ (resp., $f <_g f'$).
\fi 











==> tables.tex <==
\section{Tables}
We define the quantities shown below.

\begin{equation}
\left\{
\begin{array}{rcl}
    C(t, n)    & = & 2^{-n}\cdot\sum_{i=t}^n \binom{n}{i}  \\[0.5em]
    D(t, n)    & = & 1 - 2^{-n}\cdot \sum_{i = (n - t + 1) / 2}^{(n+t-1)/2} \binom{n}{i} \\[0.5em]
    Ball(t, n) & = & 2^{-n}\cdot \sum_{i=0}^t \binom{n}{i} \\[0.5em]
    \rho(t, n) & = & 2^{-n}\cdot \sum_{i=0}^{n-t} i\cdot \binom{n}{t+i} 
\end{array}
\right.
\end{equation}


\begin{comment}
Table \ref{tbl:c} has the thresholds for $t$ for different dimension $n$ sizes so that $C(t, n) \approx 0.01$.
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|}\hline
        $n$   & $10^3$         & $10^4$        & $10^5$      & $10^6$ \\\hline
        $t$   & $537$          & $5117$        & $50368$     & $501164$ \\\hline
    $C(t, n)$ & $0.0104635...$ & $0.009900...$ & $0.0100...$ & $0.0099826...$ \\\hline
    \end{tabular}
    \caption{Time to solve for $n = 10^5$ is about 73 seconds; time for $n=10^6$ about 25,800 seconds (more than 7 hours).}
    \label{tbl:c}
\end{table}


Table \ref{tbl:d} has the thresholds for $t$ for different dimension $n$ sizes so that $D(t, n) \approx 0.01$.
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|}\hline
        $n$   & $10^3$         & $10^4$        & $10^5$             & $10^6$ \\\hline
        $t$   & $81$           & $258$         & $815$              & ??? \\\hline 
    $D(t, n)$ & $0.0103881...$ & $0.009880...$ & $0.00995845880...$ & ??? \\\hline
    \end{tabular}
    \caption{Time to solve for $n = 10^5$ is about 22 seconds; time for $n=10^6$ is ....}
    \label{tbl:d}
\end{table}

\end{comment}




